Sound emission from oscillating bubbles trapped by the collapse of drop-impact craters

When a drop impacts a deep pool, it forms a crater which subsequently rebounds. Under certain conditions, a dimple forms at the crater bottom, which pinches off to entrap a small bubble. The oscillation of this entrapped bubble is the primary source of the underwater sound produced by rain. We use simultaneous ultra-high-speed video imaging and synchronized acoustic recording, with an immersed hydrophone, to investigate the details of the sound formation, over a range of impact Weber numbers and different dimple shapes. With frame-rates as high as 5 million fps, we can track the shape evolution of the pinched off dimple-bubble, which experiences large volumetric compression, by as much as 50%. The subsequent volume oscillations are consistent with the observed $\simeq 125$ Pa acoustic pressure amplitude, for the strongest compression. For our configuration the sound amplitude increases for smaller bubbles pinched off from the dimple. The acoustic forcing mechanism is therefore the inertial focusing of the momentum of the liquid outside the dimple, as it pinches off. The acoustic frequency agrees well with the Minnaert theory for freely oscillating spherical bubbles, of the same size. The finer details of the acoustic signal reveal an interplay between the larger dimple bubble and the tiny bubble entrapped during the initial contact between the drop and pool. For the singular dimple where no bubble is pinched off, the sound generation has a broader range of frequencies, with the tiny bubble oscillating at $\sim 100$ kHz, after being deformed by the rapid vertical retraction of the dimple below the singular jet.

==> referen.tex <==


@inproceedings{Eloh2002,
    title = {{A CCD image sensor of 1Mframes/s for continuous image capturing of 103 frames}},
    year = {2002},
    booktitle = {Solid-State Circuits Conference, 2002. Digest of Technical Papers. ISSCC. 2002 IEEE International},
    author = {Eloh, T Goji and Poggemann, D and Ruckelshausen, A and Theuwissen, A and Kreider, G and Folkerts, H-O and Mutoh, H and Kondo, Y and Maruno, H and Takubo, K},
    pages = {30--386},
    volume = {2},
    publisher = {IEEE},
    isbn = {0780373359}
}

@article{Wilson2015,
    title = {{A marine biogenic source of atmospheric ice-nucleating particles}},
    year = {2015},
    journal = {Nature},
    author = {Wilson, Theodore W and Ladino, Luis A and Alpert, Peter A and Breckels, Mark N and Brooks, Ian M and Browse, Jo and Burrows, Susannah M and Carslaw, Kenneth S and Huffman, J Alex and Judd, Christopher and Kilthau, Wendy P and Mason, Ryan H and McFiggans, Gordon and Miller, Lisa A and N{\'{a}}jera, Juan J and Polishchuk, Elena and Rae, Stuart and Schiller, Corinne L and Si, Meng and Temprado, Jesús Vergara and Whale, Thomas F and Wong, Jenny P S and Wurl, Oliver and Yakobi-Hancock, Jacqueline D and Abbatt, Jonathan P D and Aller, Josephine Y and Bertram, Allan K and Knopf, Daniel A and Murray, Benjamin J},
    pages = {234},
    volume = {525},
    publisher = {Nature Publishing Group, a division of Macmillan Publishers Limited. All Rights Reserved.},
    url = {http://dx.doi.org/10.1038/nature14986},
    doi = {10.1038/nature14986}
}

@article{Langlois2016,
  title={Toward animating water with complex acoustic bubbles},
  author={Langlois, Timothy R and Zheng, Changxi and James, Doug L},
  journal={ACM Trans. Graph. (TOG)},
  volume={35},
  number={4},
  pages={95},
  year={2016},
  publisher={ACM}
}

















@book{Worthington1908,
    title = {{A study of splashes}},
    year = {1908},
    author = {Worthington, Arthur Mason},
    publisher = {Longmans, Green, and Company}
}




@article{Smith2003,
    title = {{Air cushioning with a lubrication/inviscid balance}},
    year = {2003},
    journal = {J. Fluid Mech.},
    author = {Smith, F T and Li, L and Wu, G X},
    edition = {2003/05/13},
    pages = {291--318},
    volume = {482},
    publisher = {Cambridge University Press},
    url = {https://www.cambridge.org/core/article/air-cushioning-with-a-lubricationinviscid-balance/607E5420FE6A4F15662361B21FE71B36},
    isbn = {0022-1120},
    doi = {10.1017/S0022112003004063}
}


@article{Hicks2012,
    title = {{Air trapping at impact of a rigid sphere onto a liquid}},
    year = {2012},
    journal = {J. Fluid Mech.},
    author = {Hicks, P D and Ermanyuk, E V and Gavrilov, N V and Purvis, R},
    pages = {310--320},
    volume = {695},
    isbn = {1469-7645}
}

@article{Mills2012,
    title = {{An experimental study of Mesler entrainment on a surfactant‐covered interface: The effect of drop shape and Weber number}},
    year = {2012},
    journal = {AIChE Journal},
    author = {Mills, B H and Saylor, J R and Testik, F Y},
    number = {1},
    pages = {46--58},
    volume = {58},
    isbn = {0001-1541}
}

@article{Etoh2003,
    title = {{An image sensor which captures 100 consecutive frames at 1000000 frames/s}},
    year = {2003},
    journal = {IEEE Transactions on electron devices},
    author = {Etoh, T Goji and Poggemann, Dirk and Kreider, Greg and Mutoh, Hideki and Theuwissen, Albert J P and Ruckelshausen, Arno and Kondo, Yasushi and Maruno, Hiromasa and Takubo, Kenji and Soya, Hideki},
    number = {1},
    pages = {144--151},
    volume = {50},
    isbn = {0018-9383}
}

@article{Morton2000,
    title = {{An investigation of the flow regimes resulting from splashing drops}},
    year = {2000},
    journal = {Phys. Fluids},
    author = {Morton, David and Rudman, Murray and Jong-Leng, Liow},
    number = {4},
    pages = {747--763},
    volume = {12},
    isbn = {1070-6631}
}

@article{Beilharz2015,
    title = {{Antibubbles and fine cylindrical sheets of air}},
    year = {2015},
    journal = {J. Fluid Mech.},
    author = {Beilharz, D and Guyon, A and Li, E Q and Thoraval, M-J and Thoroddsen, Sigurdur T},
    pages = {87--115},
    volume = {779},
    isbn = {0022-1120}
}

@article{Gordillo2011,
    title = {{Asymptotic behavior of a retracting two-dimensional fluid sheet}},
    year = {2011},
    journal = {Phys. Fluids},
    author = {Gordillo, Leonardo and Agbaglah, Gilou and Duchemin, Laurent and Josserand, Christophe},
    number = {12},
    pages = {122101},
    volume = {23},
    isbn = {1070-6631}
}



@article{Esmailizadeh1986,
    title = {{Bubble entrainment with drops}},
    year = {1986},
    journal = {Journal of colloid and interface science},
    author = {Esmailizadeh, Ladan and Mesler, Russell},
    number = {2},
    pages = {561--574},
    volume = {110},
    isbn = {0021-9797}
}


@article{Lohse2019,
  title={Deep pool water-impacts of viscous oil droplets},
  author={Jain, Utkarsh and Jalaal, Maziyar and Lohse, Detlef and van der Meer, Devaraj},
  journal={Soft Matter},
  volume={15},
  number={23},
  pages={4629--4638},
  year={2019},
  publisher={Royal Society of Chemistry}
}


@article{Marston2011,
    title = {{Bubble entrapment during sphere impact onto quiescent liquid surfaces}},
    year = {2011},
    journal = {J. Fluid Mech.},
    author = {Marston, J O and Vakarelski, Ivan Uriev and Thoroddsen, Sigurdur T},
    pages = {660--670},
    volume = {680},
    isbn = {1469-7645}
}

@inproceedings{Liow2007,
    title = {{Bubble entrapment mechanisms during the impact of a water drop}},
    year = {2007},
    booktitle = {16th Australasian Fluid Mechanics Conference (AFMC)},
    author = {Liow, J L and Cole, D E},
    pages = {866--869},
    publisher = {School of Engineering, The University of Queensland},
    isbn = {1864998946}
}

@article{Ray2012,
    title = {{Bubble pinch-off and scaling during liquid drop impact on liquid pool}},
    year = {2012},
    journal = {Phys. Fluids},
    author = {Ray, Bahni and Biswas, Gautam and Sharma, Ashutosh},
    number = {8},
    pages = {82108},
    volume = {24},
    publisher = {American Institute of Physics},
    url = {https://doi.org/10.1063/1.4746793},
    isbn = {1070-6631},
    doi = {10.1063/1.4746793}
}

@article{Lhuissier2012,
    title = {{Bursting bubble aerosols}},
    year = {2012},
    journal = {J. Fluid Mech.},
    author = {Lhuissier, H and Villermaux, E},
    edition = {2011/11/18},
    pages = {5--44},
    volume = {696},
    publisher = {Cambridge University Press},
    url = {https://www.cambridge.org/core/article/bursting-bubble-aerosols/33D700585872DF6B9A50030FD7FCD0E1},
    isbn = {0022-1120},
    doi = {10.1017/jfm.2011.418}
}

@article{Elmore2001,
    title = {{Cavity and flow measurements of reproducible bubble entrainment following drop impacts}},
    year = {2001},
    journal = {Experiments in Fluids},
    author = {Elmore, P A and Chahine, G L and Oguz, H N},
    number = {6},
    pages = {664--673},
    volume = {31},
    isbn = {0723-4864}
}

@article{Thoraval2013a,
    title = {{Contraction of an air disk caught between two different liquids}},
    year = {2013},
    journal = {Phys. Rev. E},
    author = {Thoraval, M-J and Thoroddsen, Sigurdur T},
    number = {6},
    pages = {61001},
    volume = {88}
}

@article{Engel1966,
    title = {{Crater depth in fluid impacts}},
    year = {1966},
    journal = {Journal of Applied Physics},
    author = {Engel, Olive G},
    number = {4},
    pages = {1798--1808},
    volume = {37},
    isbn = {0021-8979}
}

@article{Bisighini2010,
    title = {{Crater evolution after the impact of a drop onto a semi-infinite liquid target}},
    year = {2010},
    journal = {Phys. Rev. E},
    author = {Bisighini, Alfio and Cossali, Gianpietro E and Tropea, Cameron and Roisman, Ilia V},
    number = {3},
    pages = {36319},
    volume = {82},
    publisher = {American Physical Society},
    url = {https://link.aps.org/doi/10.1103/PhysRevE.82.036319},
    doi = {10.1103/PhysRevE.82.036319}
}

@article{Thoroddsen2006,
    title = {{Crown breakup by Marangoni instability}},
    year = {2006},
    journal = {J. Fluid Mech.},
    author = {Thoroddsen, S T and Etoh, T Goji and Takehara, K},
    pages = {63--72},
    volume = {557},
    isbn = {1469-7645}
}

@inproceedings{Marston2014,
    title = {{Crown sealing and buckling instability during sphere impact}},
    year = {2014},
    booktitle = {APS Division of Fluid Dynamics Meeting Abstracts},
    author = {Marston, Jeremy and Truscott, Tadd and Mansoor, Mohammad and Thoroddsen, Sigurdur}
}

@article{Marston2016,
    title = {{Crown sealing and buckling instability during water entry of spheres}},
    year = {2016},
    journal = {J. Fluid Mech.},
    author = {Marston, J O and Truscott, T T and Speirs, N B and Mansoor, Mohammad M and Thoroddsen, Sigurdur T},
    pages = {506--529},
    volume = {794},
    isbn = {0022-1120}
}

@article{Bird2010,
    title = {{Daughter bubble cascades produced by folding of ruptured thin films}},
    year = {2010},
    journal = {Nature},
    author = {Bird, James C and de Ruiter, Riëlle and Courbin, Laurent and Stone, Howard A},
    pages = {759},
    volume = {465},
    publisher = {Nature Publishing Group, a division of Macmillan Publishers Limited. All Rights Reserved.},
    url = {http://dx.doi.org/10.1038/nature09069},
    doi = {10.1038/nature09069
https://www.nature.com/articles/nature09069{\#}supplementary-information}
}

@article{Wang2013,
    title = {{Do we understand the bubble formation by a single drop impacting upon liquid surface?}},
    year = {2013},
    journal = {Phys. Fluids},
    author = {Wang, An-Bang and Kuan, Chen-Chi and Tsai, Pei-Hsun},
    number = {10},
    pages = {101702},
    volume = {25},
    isbn = {1070-6631}
}

@article{Lhuissier2013,
    title = {{Drop Fragmentation at Impact onto a Bath of an Immiscible Liquid}},
    year = {2013},
    journal = {Phys. Rev. Lett.},
    author = {Lhuissier, H and Sun, C and Prosperetti, A and Lohse, D},
    number = {26},
    pages = {264503},
    volume = {110},
    publisher = {American Physical Society},
    url = {https://link.aps.org/doi/10.1103/PhysRevLett.110.264503},
    doi = {10.1103/PhysRevLett.110.264503}
}

@article{Lhuissier2013a,
    title = {{Drop Fragmentation at Impact onto a Bath of an Immiscible Liquid}},
    year = {2013},
    author = {Lhuissier, H and Sun, C and Prosperetti, A and Lohse, D},
    url = {https://journals.aps.org/prl/pdf/10.1103/PhysRevLett.110.264503},
    doi = {10.1103/PhysRevLett.110.264503}
}

@article{Thoraval2013,
    title = {{Drop impact entrapment of bubble rings}},
    year = {2013},
    journal = {J. Fluid Mech.},
    author = {Thoraval, M-J and Takehara, K and Etoh, T G and Thoroddsen, Sigurdur T},
    pages = {234--258},
    volume = {724},
    isbn = {0022-1120}
}

@article{Agbaglah2015,
    title = {{Drop impact into a deep pool: vortex shedding and jet formation}},
    year = {2015},
    journal = {J. Fluid Mech.},
    author = {Agbaglah, Gilou and Thoraval, M-J and Thoroddsen, Sigurdur T and Zhang, Li V and Fezzaa, Kamel and Deegan, Robert D},
    volume = {764},
    isbn = {0022-1120}
}

@article{Josserand2016,
    title = {{Drop impact on a solid surface}},
    year = {2016},
    journal = {Annu. Rev. Fluid Mech.},
    author = {Josserand, C and Thoroddsen, Sigurdur T},
    pages = {365--391},
    volume = {48},
    isbn = {0066-4189}
}

@article{Xu2005,
    title = {{Drop Splashing on a Dry Smooth Surface}},
    year = {2005},
    journal = {Phys. Rev. Lett.},
    author = {Xu, Lei and Zhang, Wendy W and Nagel, Sidney R},
    number = {18},
    pages = {184505},
    volume = {94},
    publisher = {American Physical Society},
    url = {https://link.aps.org/doi/10.1103/PhysRevLett.94.184505}
}

@book{Rein2014,
    title = {{Drop-surface interactions}},
    year = {2014},
    author = {Rein, Martin},
    volume = {456},
    publisher = {Springer},
    isbn = {3709125944}
}

@article{Castillo-Orozco2015,
    title = {{Droplet impact on deep liquid pools: Rayleigh jet to formation of secondary droplets}},
    year = {2015},
    journal = {Phys. Rev. E},
    author = {Castillo-Orozco, Eduardo and Davanlou, Ashkan and Choudhury, Pretam K and Kumar, Ranganathan},
    number = {5},
    pages = {53022},
    volume = {92}
}

@article{Deike2018,
    title = {{Dynamics of jets produced by bursting bubbles}},
    year = {2018},
    journal = {Phys. Rev. Fluids},
    author = {Deike, Luc and Ghabache, Elisabeth and Liger-Belair, Gérard and Das, Arup K and Zaleski, Stéphane and Popinet, Stéphane and S{\'{e}}on, Thomas},
    number = {1},
    pages = {13603},
    volume = {3},
    publisher = {American Physical Society},
    url = {https://link.aps.org/doi/10.1103/PhysRevFluids.3.013603},
    doi = {10.1103/PhysRevFluids.3.013603}
}

@inproceedings{Thoraval2010,
    title = {{Dynamics of the ejecta sheets generated by a drop impact}},
    year = {2010},
    booktitle = {APS Division of Fluid Dynamics Meeting Abstracts},
    author = {Thoraval, Marie-Jean and Thoroddsen, Sigurdur T}
}

@article{Yang2018,
    title = {{Economic assessment of carbon capture by minichannel absorbers}},
    year = {2018},
    journal = {AIChE Journal},
    author = {Yang, Z. and Khan, T.S. and Alshehhi, M. and AlWahedi, Y.F.},
    number = {2},
    volume = {64},
    doi = {10.1002/aic.15919},
    issn = {15475905},
    keywords = {CO  capture 2, CO  loading 2, absorption, diethanolamine, economic analysis, minichannel}
}

@article{Yang2018b,
    title = {{Economic assessment of carbon capture by minichannel absorbers}},
    year = {2018},
    journal = {AIChE Journal},
    author = {Yang, Ziqiang and Khan, Tariq S. and Alshehhi, Mohamed and AlWahedi, Yasser F.},
    number = {2},
    month = {2},
    pages = {620--631},
    volume = {64},
    publisher = {John Wiley {\&} Sons, Ltd},
    url = {http://doi.wiley.com/10.1002/aic.15919},
    doi = {10.1002/aic.15919},
    issn = {00011541},
    keywords = {CO2 capture, CO2 loading, absorption, diethanolamine, economic analysis, minichannel}
}

@article{Okawa2008,
    title = {{Effect of impingement angle on the outcome of single water drop impact onto a plane water surface}},
    year = {2008},
    journal = {Experiments in Fluids},
    author = {Okawa, Tomio and Shiraishi, Takuya and Mori, Toshiaki},
    number = {2},
    pages = {331--339},
    volume = {44},
    isbn = {0723-4864}
}

@article{Seon2017,
    title = {{Effervescence in champagne and sparkling wines: From bubble bursting to droplet evaporation}},
    year = {2017},
    journal = {The European Physical Journal Special Topics},
    author = {S{\'{e}}on, Thomas and Liger-Belair, Gérard},
    number = {1},
    pages = {117--156},
    volume = {226},
    isbn = {1951-6355}
}

@article{Zhang2012,
    title = {{Evolution of the ejecta sheet from the impact of a drop with a deep pool}},
    year = {2012},
    journal = {J. Fluid Mech.},
    author = {Zhang, L V and Toole, J and Fezzaa, K and Deegan, R D},
    pages = {5--15},
    volume = {690},
    isbn = {1469-7645}
}

@article{Castrejon-Pita2012,
    title = {{Experimental observation of von K{\textbackslash}'arm{\textbackslash}'an vortices during drop impact}},
    year = {2012},
    journal = {Phys. Rev. E},
    author = {Castrej{\'{o}}n-Pita, A A and Castrej{\'{o}}n-Pita, J R and Hutchings, I M},
    number = {4},
    pages = {45301},
    volume = {86},
    publisher = {American Physical Society},
    url = {https://link.aps.org/doi/10.1103/PhysRevE.86.045301},
    doi = {10.1103/PhysRevE.86.045301}
}

@article{Saylor2012,
    title = {{Experimental study of the role of the Weber and capillary numbers on Mesler entrainment}},
    year = {2012},
    journal = {AIChE Journal},
    author = {Saylor, John R and Bounds, Garrett D},
    number = {12},
    pages = {3841--3851},
    volume = {58},
    publisher = {Wiley-Blackwell},
    url = {https://doi.org/10.1002/aic.13764},
    isbn = {0001-1541},
    doi = {10.1002/aic.13764},
    keywords = {bubble phenomena, fluid mechanics, interfacial processes}
}


@article{Thoroddsen2007a,
    title = {{Experiments on bubble pinch-off}},
    year = {2007},
    journal = {Phys. Fluids},
    author = {Thoroddsen, S T and Etoh, T G and Takehara, K},
    number = {4},
    pages = {42101},
    volume = {19},
    isbn = {1070-6631}
}

@inproceedings{Aljedaani2016,
    title = {{Experiments on the breakup of drop-impact crowns by Marangoni holes}},
    year = {2016},
    booktitle = {APS Meeting Abstracts},
    author = {Aljedaani, Abdulrahman and Wang, C L and Jetly, A and Li, E Q and Thoroddsen, S T}
}

@book{Edgerton1954,
    title = {{Flash!: Seeing the unseen by ultra high-speed photography}},
    year = {1954},
    author = {Edgerton, Harold Eugene and Killian, James Rhyne},
    publisher = {CT Branford Co.}
}

@article{Chapman1967,
    title = {{Formation of vortex rings from falling drops}},
    year = {1967},
    journal = {J. Fluid Mech.},
    author = {Chapman, David S and Critchlow, P R},
    number = {1},
    pages = {177--185},
    volume = {29},
    isbn = {1469-7645}
}

@article{Terwagne2010,
    title = {{From a bouncing compound drop to a double emulsion}},
    year = {2010},
    journal = {Langmuir},
    author = {Terwagne, D and Gilet, T and Vandewalle, N and Dorbolo, S},
    edition = {2010/05/25},
    number = {14},
    pages = {11680--11685},
    volume = {26},
    url = {https://www.ncbi.nlm.nih.gov/pubmed/20491493},
    isbn = {1520-5827 (Electronic)
0743-7463 (Linking)},
    doi = {10.1021/la101096q},
    pmid = {20491493}
}

@article{Gekle2010,
    title = {{Generation and breakup of Worthington jets after cavity collapse. Part 1. Jet formation}},
    year = {2010},
    journal = {J. Fluid Mech.},
    author = {Gekle, Stephan and Gordillo, J M},
    pages = {293--330},
    volume = {663},
    isbn = {1469-7645}
}

@article{Gordillo2010,
    title = {{Generation and breakup of Worthington jets after cavity collapse. Part 2. Tip breakup of stretched jets}},
    year = {2010},
    journal = {J. Fluid Mech.},
    author = {Gordillo, J M and Gekle, Stephan},
    pages = {331--346},
    volume = {663},
    isbn = {1469-7645}
}

@article{Jetly2019,
    title = {{Giant drag reduction on Leidenfrost spheres evaluated from extended free-fall trajectories}},
    year = {2019},
    journal = {Experimental Thermal and Fluid Science},
    author = {Jetly, Aditya and Vakarelski, Ivan U. and Yang, Ziqiang and Thoroddsen, Sigurdur T.},
    month = {4},
    pages = {181--188},
    volume = {102},
    publisher = {Elsevier},
    url = {https://www.sciencedirect.com/science/article/pii/S0894177718316662},
    doi = {10.1016/J.EXPTHERMFLUSCI.2018.11.010},
    issn = {0894-1777}
}

@incollection{Langley2018,
    title = {{High-Speed Interferometry Under Impacting Drops}},
    year = {2018},
    booktitle = {The Micro-World Observed by Ultra High-Speed Cameras},
    author = {Langley, Kenneth R and Li, Er Q and Thoroddsen, Sigurdur T},
    pages = {321--341},
    publisher = {Springer}
}

@article{Gulyaev2013,
    title = {{Hollow droplets impacting onto a solid surface}},
    year = {2013},
    journal = {Experiments in Fluids},
    author = {Gulyaev, I P and Solonenko, O P},
    number = {1},
    pages = {1432},
    volume = {54},
    isbn = {0723-4864}
}

@article{Semenov2015,
    title = {{Impact of liquids with different densities}},
    year = {2015},
    journal = {J. Fluid Mech.},
    author = {Semenov, Y  A and Wu, G  X and Korobkin, A  A},
    edition = {2015/01/30},
    pages = {5--27},
    volume = {766},
    publisher = {Cambridge University Press},
    url = {https://www.cambridge.org/core/article/impact-of-liquids-with-different-densities/AA6D58EB9D2EEA3BCB1F1C9549A3BD3F},
    isbn = {0022-1120},
    doi = {10.1017/jfm.2015.8}
}

@inproceedings{Langley2016,
    title = {{Impact of ultra-viscous drops on a smooth solid surface}},
    year = {2016},
    booktitle = {APS Meeting Abstracts},
    author = {Langley, Kenneth and Li, E Q and Thoroddsen, S T}
}

@article{Worthington1897,
    title = {{Impact with a liquid surface, studied by the aid of instantaneous photography}},
    year = {1897},
    journal = {Philosophical Transactions of the Royal Society of London. Series A, Containing Papers of a Mathematical or Physical Character},
    author = {Worthington, Arthur Mason and Cole, Reginald Sorrè},
    pages = {137--148},
    volume = {189},
    isbn = {0264-3952}
}

@article{Worthington1897a,
    title = {{Impact with a Liquid Surface, Studied by the Aid of Instantaneous Photography}},
    year = {1897},
    journal = {Philosophical Transactions of the Royal Society A: Mathematical, Physical and Engineering Sciences},
    author = {Worthington, A. M. and Cole, R. S.},
    number = {0},
    month = {1},
    pages = {137--148},
    volume = {189},
    url = {http://rsta.royalsocietypublishing.org/cgi/doi/10.1098/rsta.1897.0005},
    doi = {10.1098/rsta.1897.0005},
    issn = {1364-503X}
}

@article{Worthington1897b,
    title = {{Impact with a Liquid Surface, Studied by the Aid of Instantaneous Photography}},
    year = {1897},
    journal = {Philosophical Transactions of the Royal Society A: Mathematical, Physical and Engineering Sciences},
    author = {Worthington, A. M. and Cole, R. S.},
    number = {0},
    pages = {137--148},
    volume = {189},
    url = {http://rsta.royalsocietypublishing.org/cgi/doi/10.1098/rsta.1897.0005},
    isbn = {0264-3952},
    doi = {10.1098/rsta.1897.0005},
    issn = {1364-503X}
}

@article{Bouwhuis2015,
    title = {{Initial surface deformations during impact on a liquid pool}},
    year = {2015},
    journal = {J. Fluid Mech.},
    author = {Bouwhuis, Wilco and Hendrix, Maurice H W and van der Meer, Devaraj and Snoeijer, Jacco H},
    pages = {503--519},
    volume = {771},
    isbn = {0022-1120}
}

@article{Bouwhuis2015a,
    title = {{Initial surface deformations during impact on a liquid pool}},
    year = {2015},
    journal = {J. Fluid Mech.},
    author = {Bouwhuis, Wilco and Hendrix, Maurice H W and van der Meer, Devaraj and Snoeijer, Jacco H},
    pages = {503--519},
    volume = {771},
    isbn = {0022-1120}
}

@article{Yamamoto2018,
    title = {{Initiation of the Worthington jet on the droplet impact}},
    year = {2018},
    journal = {Applied Physics Letters},
    author = {Yamamoto, Ken and Motosuke, Masahiro and Ogata, Satoshi},
    number = {9},
    pages = {93701},
    volume = {112},
    isbn = {0003-6951}
}

@article{Fujimatsu2003,
    title = {{Interfacial deformation between an impacting water drop and a silicone-oil surface}},
    year = {2003},
    journal = {Journal of colloid and interface science},
    author = {Fujimatsu, Takahiro and Fujita, Hideomi and Hirota, Masafumi and Okada, Osamu},
    number = {1},
    pages = {212--220},
    volume = {264},
    isbn = {0021-9797}
}

@article{Michon2017,
    title = {{Jet dynamics post drop impact on a deep pool}},
    year = {2017},
    journal = {Phys. Rev. Fluids},
    author = {Michon, Guy-Jean and Josserand, Christophe and S{\'{e}}on, Thomas},
    number = {2},
    pages = {23601},
    volume = {2}
}

@article{Duchemin2002,
    title = {{Jet formation in bubbles bursting at a free surface}},
    year = {2002},
    journal = {Phys. Fluids},
    author = {Duchemin, Laurent and Popinet, Stéphane and Josserand, Christophe and Zaleski, Stéphane},
    number = {9},
    pages = {3000--3008},
    volume = {14},
    isbn = {1070-6631}
}

@article{Zou2012,
    title = {{Large bubble entrapment during drop impacts on a restricted liquid surface}},
    year = {2012},
    journal = {Phys. Fluids},
    author = {Zou, Jun and Ji, Chen and Yuan, BaoGang and Ren, YuLiang and Ruan, XiaoDong and Fu, Xin},
    number = {5},
    pages = {57101},
    volume = {24},
    isbn = {1070-6631}
}

@article{Dong2019,
    title = {{Laser induced fluorescence studies on the distribution of surfactants during drop/ interface coalescence}},
    year = {2019},
    journal = {Phys. Fluids},
    author = {Dong, Teng and Weheliye, Weheliye Hashi and Angeli, Panagiota},
    number = {September 2018},
    pages = {12106},
    volume = {31},
    url = {https://doi.org/10.1063/1.5059554%0Ahttps://doi.org/10.1063/1.5059554},
    doi = {10.1063/1.5059554},
    issn = {1070-6631}
}

@article{Knelman1954,
    title = {{Mechanism of the bursting of bubbles}},
    year = {1954},
    journal = {Nature},
    author = {Knelman, F and Dombrowski, N and Newitt, D M},
    number = {4397},
    pages = {261},
    volume = {173},
    isbn = {1476-4687}
}

@article{Thoroddsen2012a,
    title = {{Micro-bubble morphologies following drop impacts onto a pool surface}},
    year = {2012},
    journal = {J. Fluid Mech.},
    author = {Thoroddsen, S T and Thoraval, M J and Takehara, K and Etoh, T G},
    chapter = {469},
    pages = {469--479},
    volume = {708},
    isbn = {0022-1120
1469-7645},
    doi = {10.1017/jfm.2012.319}
}

@article{Thoroddsen2012,
    title = {{Micro-bubble morphologies following drop impacts onto a pool surface}},
    year = {2012},
    journal = {J. Fluid Mech.},
    author = {Thoroddsen, Sigurdur T and Thoraval, M-J and Takehara, K and Etoh, T G},
    pages = {469--479},
    volume = {708},
    isbn = {1469-7645}
}

@article{Thoroddsen2007,
    title = {{Microjetting from wave focusing on oscillating drops}},
    year = {2007},
    journal = {Phys. Fluids},
    author = {Thoroddsen, S T and Etoh, T G and Takehara, K},
    number = {5},
    pages = {52101},
    volume = {19},
    isbn = {1070-6631}
}

@article{Walker2015,
    title = {{Multiphase flow of miscible liquids: jets and drops}},
    year = {2015},
    journal = {Experiments in Fluids},
    author = {Walker, Travis W and Logia, Alison N and Fuller, Gerald G},
    number = {5},
    pages = {106},
    volume = {56},
    isbn = {0723-4864}
}

@article{Worthington1882,
    title = {{On impact with a liquid surface}},
    year = {1882},
    journal = {Proceedings of the Royal Society of London (1854-1905)},
    author = {Worthington, A},
    number = {-1},
    pages = {217--230},
    volume = {34},
    url = {papers://7652351a-a335-41fa-8308-0f4f73f54070/Paper/p659},
    isbn = {03701662},
    doi = {10.1098/rspl.1882.0035},
    issn = {0370-1662}
}

@article{Fedorchenko2004,
    title = {{On some common features of drop impact on liquid surfaces}},
    year = {2004},
    journal = {Phys. Fluids},
    author = {Fedorchenko, Alexander I and Wang, An-Bang},
    number = {5},
    pages = {1349--1365},
    volume = {16},
    isbn = {1070-6631}
}

@article{Brenner1999,
    title = {{On the bursting of viscous films}},
    year = {1999},
    journal = {Phys. Fluids},
    author = {Brenner, Michael P and Gueyffier, Denis},
    number = {3},
    pages = {737--739},
    volume = {11},
    isbn = {1070-6631}
}


@article{Ghabache2014,
    title = {{On the physics of fizziness: How bubble bursting controls droplets ejection}},
    year = {2014},
    journal = {Phys. Fluids},
    author = {Ghabache, Elisabeth and Antkowiak, Arnaud and Josserand, Christophe and S{\'{e}}on, Thomas},
    number = {12},
    pages = {121701},
    volume = {26},
    isbn = {1070-6631}
}

@article{Rayleigh1889,
    title = {{On the tension of recently formed liquid surfaces}},
    year = {1889},
    journal = {Proceedings of the Royal Society of London},
    author = {Rayleigh, Lord},
    pages = {281--287},
    volume = {47},
    isbn = {0370-1662}
}

@article{Lee2015,
    title = {{Origin and dynamics of vortex rings in drop splashing}},
    year = {2015},
    journal = {Nature communications},
    author = {Lee, Ji San and Park, Su Ji and Lee, Jun Ho and Weon, Byung Mook and Fezzaa, Kamel and Je, Jung Ho},
    pages = {8187},
    volume = {6},
    publisher = {The Author(s)},
    url = {http://dx.doi.org/10.1038/ncomms9187},
    doi = {10.1038/ncomms9187
https://www.nature.com/articles/ncomms9187{\#}supplementary-information}
}

@article{Martin1993,
    title = {{Phenomena of liquid drop impact on solid and liquid surfaces}},
    year = {1993},
    journal = {Fluid Dynamics Research},
    author = {Martin, Rein},
    number = {2},
    pages = {61},
    volume = {12},
    url = {http://stacks.iop.org/1873-7005/12/i=2/a=A01},
    isbn = {1873-7005}
}

@article{Eggers2008,
    title = {{Physics of liquid jets}},
    year = {2008},
    journal = {Reports on Progress in Physics},
    author = {Eggers, Jens and Villermaux, Emmanuel},
    number = {3},
    pages = {36601},
    volume = {71},
    isbn = {0034-4885}
}

@article{Ray2015,
    title = {{Regimes during liquid drop impact on a liquid pool}},
    year = {2015},
    journal = {J. Fluid Mech.},
    author = {Ray, Bahni and Biswas, Gautam and Sharma, Ashutosh},
    edition = {2015/03/10},
    pages = {492--523},
    volume = {768},
    publisher = {Cambridge University Press},
    url = {https://www.cambridge.org/core/article/regimes-during-liquid-drop-impact-on-a-liquid-pool/0C7AFF1DBEAA106FE9C7A15E75A007C4},
    isbn = {0022-1120},
    doi = {10.1017/jfm.2015.108}
}

@article{Ganan-Calvo2017,
    title = {{Revision of bubble bursting: universal scaling laws of top jet drop size and speed}},
    year = {2017},
    journal = {Phys. Rev. Lett.},
    author = {Ga{\~{n}}{\'{a}}n-Calvo, Alfonso M},
    number = {20},
    pages = {204502},
    volume = {119}
}

@article{Li2014a,
    title = {{Satellite formation during bubble transition through an interface between immiscible liquids}},
    year = {2014},
    journal = {J. Fluid Mech.},
    author = {Li, E Q and Al-Otaibi, S A and Vakarelski, Ivan Uriev and Thoroddsen, Sigurdur T},
    volume = {744},
    isbn = {0022-1120}
}

@article{Li2014,
    title = {{Satellite formation during bubble transition through an interface between immiscible liquids}},
    year = {2014},
    journal = {J. Fluid Mech.},
    author = {Li, E Q and Al-Otaibi, S A and Vakarelski, Ivan Uriev and Thoroddsen, Sigurdur T},
    volume = {744},
    isbn = {0022-1120}
}

@article{Weiss1999,
    title = {{Single drop impact onto liquid films: neck distortion, jetting, tiny bubble entrainment, and crown formation}},
    year = {1999},
    journal = {J. Fluid Mech.},
    author = {Weiss, Daniel A and Yarin, Alexander L},
    pages = {229--254},
    volume = {385},
    isbn = {1469-7645}
}

@article{Bartolo2006,
    title = {{Singular jets and bubbles in drop impact}},
    year = {2006},
    journal = {Phys. Rev. Lett.},
    author = {Bartolo, Denis and Josserand, Christophe and Bonn, Daniel},
    number = {12},
    pages = {124501},
    volume = {96}
}




@article{Zeff2000,
    title = {{Singularity dynamics in curvature collapse and jet eruption on a fluid surface}},
    year = {2000},
    journal = {Nature},
    author = {Zeff, Benjamin W and Kleber, Benjamin and Fineberg, Jay and Lathrop, Daniel P},
    number = {6768},
    pages = {401},
    volume = {403},
    isbn = {1476-4687}
}

@article{Lee2011,
    title = {{Size limits the formation of liquid jets during bubble bursting}},
    year = {2011},
    journal = {Nature communications},
    author = {Lee, Ji San and Weon, Byung Mook and Park, Su Ji and Je, Jung Ho and Fezzaa, Kamel and Lee, Wah-Keat},
    pages = {367},
    volume = {2},
    publisher = {The Author(s)},
    url = {http://dx.doi.org/10.1038/ncomms1369},
    doi = {10.1038/ncomms1369
https://www.nature.com/articles/ncomms1369{\#}supplementary-information}
}

@article{Lee2011a,
    title = {{Size limits the formation of liquid jets during bubble bursting}},
    year = {2011},
    author = {Lee, Ji San and Weon, Byung Mook and Park, Su Ji and Je, Jung Ho and Fezzaa, Kamel and Lee, Wah-Keat},
    pages = {367},
    volume = {2},
    publisher = {The Author(s)},
    url = {http://dx.doi.org/10.1038/ncomms1369},
    doi = {10.1038/ncomms1369
https://www.nature.com/articles/ncomms1369{\#}supplementary-information}
}

@article{Ghabache2016,
    title = {{Size of the top jet drop produced by bubble bursting}},
    year = {2016},
    journal = {Phys. Rev. Fluids},
    author = {Ghabache, Elisabeth and S{\'{e}}on, Thomas},
    number = {5},
    pages = {51901},
    volume = {1}
}

@article{Rodriguez1985,
    title = {{Some drops don't splash}},
    year = {1985},
    journal = {Journal of colloid and interface science},
    author = {Rodriguez, Francisco and Mesler, Russell},
    number = {2},
    pages = {347--352},
    volume = {106},
    isbn = {0021-9797}
}

@article{Murphy2015,
    title = {{Splash behaviour and oily marine aerosol production by raindrops impacting oil slicks}},
    year = {2015},
    journal = {J. Fluid Mech.},
    author = {Murphy, David W and Li, Cheng and d’Albignac, Vincent and Morra, David and Katz, Joseph},
    pages = {536--577},
    volume = {780},
    isbn = {0022-1120}
}

@article{Leng2001,
    title = {{Splash formation by spherical drops}},
    year = {2001},
    journal = {J. Fluid Mech.},
    author = {Leng, Liow Jong},
    pages = {73--105},
    volume = {427},
    isbn = {1469-7645}
}

@article{Semenov2013,
    title = {{Splash jet generated by collision of two liquid wedges}},
    year = {2013},
    journal = {J. Fluid Mech.},
    author = {Semenov, Y A and Wu, G X and Oliver, J M},
    edition = {2013/11/20},
    pages = {132--145},
    volume = {737},
    publisher = {Cambridge University Press},
    url = {https://www.cambridge.org/core/article/splash-jet-generated-by-collision-of-two-liquid-wedges/1C43DD3B879766208C3455E536A21F02},
    isbn = {0022-1120},
    doi = {10.1017/jfm.2013.529}
}

@article{Hobbs1967,
    title = {{Splashing of a water drop}},
    year = {1967},
    journal = {Science},
    author = {Hobbs, P V and Kezweeny, A J},
    number = {3766},
    pages = {1112--1114},
    volume = {155},
    isbn = {0036-8075}
}

@article{Xu2007,
    title = {{Splashing of liquids: Interplay of surface roughness with surrounding gas}},
    year = {2007},
    journal = {Phys. Rev. E},
    author = {Xu, Lei and Barcos, Loreto and Nagel, Sidney R},
    number = {6},
    pages = {66311},
    volume = {76}
}

@article{Edgerton1977,
    title = {{Stopping Time: The Photographs of Harold Edgerton (Abrams, New York, 1977)}},
    year = {1977},
    author = {Edgerton, Harold and Jussim, Estelle and Kayafas, Gus}
}

@article{Hao2015,
    title = {{Superhydrophobic-like tunable droplet bouncing on slippery liquid interfaces}},
    year = {2015},
    journal = {Nature communications},
    author = {Hao, Chonglei and Li, Jing and Liu, Yuan and Zhou, Xiaofeng and Liu, Yahua and Liu, Rong and Che, Lufeng and Zhou, Wenzhong and Sun, Dong and Li, Lawrence and Xu, Lei and Wang, Zuankai},
    pages = {7986},
    volume = {6},
    publisher = {The Author(s)},
    url = {http://dx.doi.org/10.1038/ncomms8986},
    doi = {10.1038/ncomms8986
https://www.nature.com/articles/ncomms8986{\#}supplementary-information}
}

@article{Tomita2007,
    title = {{Surface breakup and air bubble formation by drop impact in the irregular entrainment region}},
    year = {2007},
    journal = {J. Fluid Mech.},
    author = {Tomita, Y and Saito, T and Ganbara, S},
    pages = {131--152},
    volume = {588},
    isbn = {1469-7645}
}

@article{Richard2002,
    title = {{Surface phenomena: Contact time of a bouncing drop}},
    year = {2002},
    journal = {Nature},
    author = {Richard, Denis and Clanet, Christophe and Qu{\'{e}}r{\'{e}}, David},
    number = {6891},
    pages = {811},
    volume = {417},
    isbn = {1476-4687}
}

@article{Oguz1989,
    title = {{Surface-tension effects in the contact of liquid surfaces}},
    year = {1989},
    journal = {J. Fluid Mech.},
    author = {Oguz, Hasan N and Prosperetti, Andrea},
    pages = {149--171},
    volume = {203},
    isbn = {1469-7645}
}








@article{Thoroddsen2005,
    title = {{The air bubble entrapped under a drop impacting on a solid surface}},
    year = {2005},
    journal = {J. Fluid Mech.},
    author = {Thoroddsen, S T and Etoh, T G and Takehara, K and Ootsuka, N and Hatsuki, Y},
    pages = {203--212},
    volume = {545},
    isbn = {1469-7645}
}

@article{Medwin1992,
    title = {{The anatomy of underwater rain noise}},
    year = {1992},
    journal = {J. Acoust. Soc. Am.},
    author = {Medwin, Herman and Nystuen, Jeffrey A and Jacobus, Peter W and Ostwald, Leo H and Snyder, David E},
    number = {3},
    pages = {1613--1623},
    volume = {92},
    isbn = {0001-4966}
}

@article{Sigler1990,
    title = {{The behavior of the gas film formed upon drop impact with a liquid surface}},
    year = {1990},
    journal = {Journal of colloid and interface science},
    author = {Sigler, James and Mesler, Russell},
    number = {2},
    pages = {459--474},
    volume = {134},
    isbn = {0021-9797}
}

@article{Thoroddsen2000,
    title = {{The coalescence cascade of a drop}},
    year = {2000},
    journal = {Phys. Fluids},
    author = {Thoroddsen, S T and Takehara, K},
    number = {6},
    pages = {1265--1267},
    volume = {12},
    isbn = {1070-6631}
}

@article{Charles1960,
    title = {{The coalescence of liquid drops with flat liquid/liquid interfaces}},
    year = {1960},
    journal = {Journal of Colloid Science},
    author = {Charles, Go Eo and Mason, So Go},
    number = {3},
    pages = {236--267},
    volume = {15},
    isbn = {0095-8522}
}

@article{Hsiao1988,
    title = {{The critical Weber number for vortex and jet formation for drops impinging on a liquid pool}},
    year = {1988},
    journal = {The Phys. Fluids},
    author = {Hsiao, Mingying and Lichter, Seth and Quintero, Luis G},
    number = {12},
    pages = {3560--3562},
    volume = {31},
    isbn = {0031-9171}
}

@article{Lhuissier2011,
    title = {{The destabilization of an initially thick liquid sheet edge}},
    year = {2011},
    journal = {Phys. Fluids},
    author = {Lhuissier, Henri and Villermaux, Emmanuel},
    number = {9},
    pages = {91705},
    volume = {23},
    isbn = {1070-6631}
}



@article{Song1999,
    title = {{The formation of thick borders on an initially stationary fluid sheet}},
    year = {1999},
    journal = {Phys. Fluids},
    author = {Song, Museok and Tryggvason, Grétar},
    number = {9},
    pages = {2487--2493},
    volume = {11},
    isbn = {1070-6631}
}



@article{Prosperetti1993a,
    title = {{The impact of drops on liquid surfaces and the underwater noise of rain}},
    year = {1993},
    journal = {Annu. Rev. Fluid Mech.},
    author = {Prosperetti, Andrea and Oguz, Hasan N},
    number = {1},
    pages = {577--602},
    volume = {25},
    isbn = {0066-4189}
}

@article{Terwagne2009,
    title = {{The mayonnaise droplet}},
    year = {2009},
    journal = {Chaos},
    author = {Terwagne, D and Mack, N and Dorbolo, S and Gilet, T and Raty, J Y and Vandewalle, N},
    edition = {2010/01/12},
    number = {4},
    pages = {41105},
    volume = {19},
    url = {https://www.ncbi.nlm.nih.gov/pubmed/20059189},
    isbn = {1089-7682 (Electronic)
1054-1500 (Linking)},
    doi = {10.1063/1.3202626},
    pmid = {20059189},
    keywords = {*Algorithms, *Computer Graphics, *Computer Simulation, *Nonlinear Dynamics, Oils/*chemistry, Rheology/*methods, User-Computer Interface, Water/*chemistry}
}

@article{Deng2009,
    title = {{The phenomenon of bubble entrapment during capsule formation}},
    year = {2009},
    journal = {Journal of colloid and interface science},
    author = {Deng, Q and Anilkumar, A V and Wang, T G},
    number = {2},
    pages = {523--532},
    volume = {333},
    isbn = {0021-9797}
}

@article{Deng2007,
    title = {{The role of viscosity and surface tension in bubble entrapment during drop impact onto a deep liquid pool}},
    year = {2007},
    journal = {J. Fluid Mech.},
    author = {Deng, Q and Anilkumar, A V and Wang, T G},
    pages = {119--138},
    volume = {578},
    isbn = {1469-7645}
}

@phdthesis{Cole2007,
    title = {{The splashing morphology of liquid-liquid impacts}},
    year = {2007},
    author = {Cole, David},
    publisher = {James Cook University}
}

@article{Peck1994,
    title = {{The three‐dimensional vortex structure of an impacting water drop}},
    year = {1994},
    journal = {Phys. Fluids},
    author = {Peck, Bill and Sigurdson, Lorenz},
    number = {2},
    pages = {564--576},
    volume = {6},
    isbn = {1070-6631}
}

@article{Rein1996,
    title = {{The transitional regime between coalescing and splashing drops}},
    year = {1996},
    journal = {J. Fluid Mech.},
    author = {Rein, Martin},
    pages = {145--165},
    volume = {306},
    isbn = {1469-7645}
}

@article{Prosperetti1989,
    title = {{The underwater noise of rain}},
    year = {1989},
    journal = {Journal of Geophysical Research: Oceans},
    author = {Prosperetti, A and Crum, L A and Pumphrey, H C},
    number = {C3},
    pages = {3255--3259},
    volume = {94},
    url = {https://agupubs.onlinelibrary.wiley.com/doi/abs/10.1029/JC094iC03p03255},
    doi = {doi:10.1029/JC094iC03p03255}
}

@article{Zhao2011,
    title = {{Transition between coalescence and bouncing of droplets on a deep liquid pool}},
    year = {2011},
    journal = {International Journal of Multiphase Flow},
    author = {Zhao, He and Brunsvold, Amy and Munkejord, Svend Tollak},
    chapter = {1109},
    number = {9},
    pages = {1109--1119},
    volume = {37},
    isbn = {03019322},
    doi = {10.1016/j.ijmultiphaseflow.2011.06.007}
}

@article{Korobkin2008,
    title = {{Trapping of air in impact between a body and shallow water}},
    year = {2008},
    journal = {J. Fluid Mech.},
    author = {Korobkin, A A and Ellis, A S and Smith, F T},
    edition = {2008/09/25},
    pages = {365--394},
    volume = {611},
    publisher = {Cambridge University Press},
    url = {https://www.cambridge.org/core/article/trapping-of-air-in-impact-between-a-body-and-shallow-water/3BD13FE212FB83C8425E1321E5107807},
    isbn = {0022-1120},
    doi = {10.1017/S0022112008002899}
}

@article{Scrimger1985,
    title = {{Underwater noise caused by precipitation}},
    year = {1985},
    journal = {Nature},
    author = {Scrimger, Joseph A},
    number = {6047},
    pages = {647},
    volume = {318},
    isbn = {1476-4687}
}

@article{Pumphrey1989,
    title = {{Underwater sound produced by individual drop impacts and rainfall}},
    year = {1989},
    journal = {J. Acoust. Soc. Am.},
    author = {Pumphrey, H. C. and Crum, L A and Bjo/Rno/, L},
    number = {4},
    pages = {1518--1526},
    volume = {85},
    isbn = {0001-4966}
}

@article{Hendrix2016,
    title = {{Universal mechanism for air entrainment during liquid impact}},
    year = {2016},
    journal = {J. Fluid Mech.},
    author = {Hendrix, Maurice H W and Bouwhuis, Wilco and van der Meer, Devaraj and Lohse, Detlef and Snoeijer, Jacco H},
    pages = {708--725},
    volume = {789},
    isbn = {0022-1120}
}

@article{Chen2014,
    title = {{Viscosity effect on regular bubble entrapment during drop impact into a deep pool}},
    year = {2014},
    journal = {Chem. Eng. Sci.},
    author = {Chen, Senlin and Guo, Liejin},
    pages = {1--16},
    volume = {109},
    isbn = {0009-2509}
}

@article{Thoraval2012,
    title = {{von K{\'{a}}rm{\'{a}}n vortex street within an impacting drop}},
    year = {2012},
    journal = {Phys. Rev. Lett.},
    author = {Thoraval, Marie-Jean and Takehara, Kohsei and Etoh, Takeharu Goji and Popinet, Stéphane and Ray, Pascal and Josserand, Christophe and Zaleski, Stéphane and Thoroddsen, Sigurdur T},
    number = {26},
    pages = {264506},
    volume = {108}
}

@article{Shankar1995,
    title = {{Vortex rings generated by drops just coalescing with a pool}},
    year = {1995},
    journal = {Phys. Fluids},
    author = {Shankar, P N and Kumar, Manoj},
    number = {4},
    pages = {737--746},
    volume = {7},
    isbn = {1070-6631}
}

@incollection{Joseph1993,
    title = {{Vortex Rings of One Fluid in Another in Free Fall}},
    year = {1993},
    booktitle = {Fundamentals of Two-Fluid Dynamics},
    author = {Joseph, Daniel D and Renardy, Yuriko Y},
    pages = {288--323},
    publisher = {Springer}
}

@article{Li2017,
    title = {{Vortex-induced buckling of a viscous drop impacting a pool}},
    year = {2017},
    journal = {Phys. Rev. Fluids},
    author = {Li, Er Qiang and Beilharz, Daniel and Thoroddsen, Sigurdur T},
    number = {7},
    pages = {73602},
    volume = {2},
    publisher = {American Physical Society},
    url = {https://link.aps.org/doi/10.1103/PhysRevFluids.2.073602}
}

@article{Alchalabi2017,
    title = {{Vortex-Induced Vapor Explosion during Drop Impact on a Superheated Pool}},
    year = {2017},
    journal = {Experimental Thermal and Fluid Science},
    author = {Alchalabi, M A and Kouraytem, N and Li, E Q and Thoroddsen, Sigurdur T},
    isbn = {0894-1777}
}

@article{Thoraval2016,
    title = {{Vortex-ring-induced large bubble entrainment during drop impact}},
    year = {2016},
    journal = {Phys. Rev. E},
    author = {Thoraval, Marie-Jean and Li, Yangfan and Thoroddsen, Sigurdur T},
    number = {3},
    pages = {33128},
    volume = {93}
}

@article{Lhuissier2013DropLiquid,
    title = {{Drop Fragmentation at Impact onto a Bath of an Immiscible Liquid}},
    year = {2013},
    journal = {Phys. Rev. Lett.},
    author = {Lhuissier, H. and Sun, C. and Prosperetti, A. and Lohse, D.},
    number = {26},
    month = {6},
    pages = {264503},
    volume = {110},
    publisher = {American Physical Society},
    url = {https://link.aps.org/doi/10.1103/PhysRevLett.110.264503},
    doi = {10.1103/PhysRevLett.110.264503},
    issn = {0031-9007}
}

@article{Agbaglah2015DropFormation,
    title = {{Drop impact into a deep pool: Vortex shedding and jet formation}},
    year = {2015},
    journal = {J. Fluid Mech.},
    author = {Agbaglah, G. and Thoraval, M. J. and Thoroddsen, S. T. and Zhang, L. V. and Fezzaa, K. and Deegan, R. D.},
    isbn = {0022-1120},
    doi = {10.1017/jfm.2014.723},
    issn = {14697645},
    keywords = {breakup/coalescence, drops, drops and bubbles}
}

@article{Chen2017DropSurfaces,
    title = {{Drop impact on spherical soft surfaces}},
    year = {2017},
    journal = {Phys. Fluids},
    author = {Chen, Simeng and Bertola, Volfango},
    number = {8},
    volume = {29},
    isbn = {01956744},
    doi = {10.1063/1.4996587},
    issn = {10897666}
}

@article{Yang2018EconomicAbsorbers,
    title = {{Economic assessment of carbon capture by minichannel absorbers}},
    year = {2018},
    journal = {AIChE Journal},
    author = {Yang, Z. and Khan, T.S. and Alshehhi, M. and AlWahedi, Y.F.},
    doi = {10.1002/aic.15919},
    issn = {15475905},
    keywords = {CO  capture 2, CO  loading 2, absorption, diethanolamine, economic analysis, minichannel}
}

@article{Jetly2019GiantTrajectories,
    title = {{Giant drag reduction on Leidenfrost spheres evaluated from extended free-fall trajectories}},
    year = {2019},
    journal = {Experimental Thermal and Fluid Science},
    author = {Jetly, Aditya and Vakarelski, Ivan U. and Yang, Ziqiang and Thoroddsen, Sigurdur T.},
    doi = {10.1016/j.expthermflusci.2018.11.010},
    issn = {08941777},
    keywords = {Drag crisis, Drag reduction, Leidenfrost effect, Vapor layer}
}

@article{Gielen2017ObliquePool,
    title = {{Oblique drop impact onto a deep liquid pool}},
    year = {2017},
    journal = {Phys. Rev. Fluids},
    author = {Gielen, Marise V. and Sleutel, Pascal and Benschop, Jos and Riepen, Michel and Voronina, Victoria and Visser, Claas Willem and Lohse, Detlef and Snoeijer, Jacco H. and Versluis, Michel and Gelderblom, Hanneke},
    doi = {10.1103/PhysRevFluids.2.083602},
    issn = {2469990X},
    arxivId = {arXiv:1611.05670v1}
}



@article{1883OnSurface,
    title = {{On impact with a liquid surface}},
    year = {1883},
    journal = {Proceedings of the Royal Society of London},
    number = {220-223},
    month = {1},
    pages = {217--230},
    volume = {34},
    url = {http://www.royalsocietypublishing.org/doi/10.1098/rspl.1882.0035},
    doi = {10.1098/rspl.1882.0035},
    issn = {0370-1662}
}

@article{Worthington1882OnSurface,
    title = {{On impact with a liquid surface}},
    year = {1882},
    journal = {Proceedings of the Royal Society of London (1854-1905)},
    author = {Worthington, A},
    isbn = {03701662},
    doi = {10.1098/rspl.1882.0035},
    issn = {0370-1662}
}

@article{Worthington1882OnSurfaceb,
    title = {{On impact with a liquid surface}},
    year = {1882},
    journal = {Proceedings of the Royal Society of London (1854-1905)},
    author = {Worthington, A},
    isbn = {03701662},
    doi = {10.1098/rspl.1882.0035},
    issn = {0370-1662}
}

@article{Ganapathy2016ProcessCapture,
    title = {{Process intensification characteristics of a microreactor absorber for enhanced CO2 capture}},
    year = {2016},
    journal = {Applied Energy},
    author = {Ganapathy, Harish and Steinmayer, Sascha and Shooshtari, Amir and Dessiatoun, Serguei and Ohadi, Michael M. and Alshehhi, Mohamed},
    month = {1},
    pages = {416--427},
    volume = {162},
    url = {http://www.sciencedirect.com/science/article/pii/S0306261915012374},
    doi = {10.1016/j.apenergy.2015.10.010},
    issn = {03062619},
    keywords = {Absorption, CO2, Carbon capture, Micro-structured, Microchannel, Microreactor}
}


@article{Deka2017ThePool,
    title = {{The regime of large bubble entrapment during a single drop impact on a liquid pool}},
    year = {2017},
    journal = {Phys. Fluids},
    author = {Deka, Hiranya and Ray, Bahni and Biswas, Gautam and Dalal, Amaresh and Tsai, Pei Hsun and Wang, An Bang},
    number = {9},
    volume = {29},
    doi = {10.1063/1.4992124},
    issn = {10897666}
}

@article{Li2017Vortex-inducedPool,
    title = {{Vortex-induced buckling of a viscous drop impacting a pool}},
    year = {2017},
    journal = {Phys. Rev. Fluids},
    author = {Li, Er Qiang and Beilharz, Daniel and Thoroddsen, Sigurdur T.},
    doi = {10.1103/PhysRevFluids.2.073602},
    issn = {2469990X}
}

@misc{ZZZZZ1645745906.pdf,
    title = {{ZZZZZ1645745906.pdf}}
}

@misc{ZZZZZ2638494627.pdf,
    title = {{ZZZZZ2638494627.pdf}}
}

@article{mills2012experimental,
  title={An experimental study of Mesler entrainment on a surfactant-covered interface: The effect of drop shape and Weber number},
  author={Mills, BH and Saylor, JR and Testik, FY},
  journal={AIChE Journal},
  volume={58},
  number={1},
  pages={46--58},
  year={2012},
  publisher={Wiley Online Library}
}









@article{deane2002,
  title={Scale dependence of bubble creation mechanisms in breaking waves},
  author={Deane, Grant B and Stokes, M Dale},
  journal={Nature},
  volume={418},
  number={6900},
  pages={839--844},
  year={2002},
  publisher={Nature Publishing Group}
}
{"mode":"full","isActive":false}


@article{melville1996,
  title={The role of surface-wave breaking in air-sea interaction},
  author={Melville, W Kendall},
  journal={Annu. Rev. Fluid Mech.},
  volume={28},
  number={1},
  pages={279--321},
  year={1996},
  publisher={Annual Reviews 4139 El Camino Way, PO Box 10139, Palo Alto, CA 94303-0139, USA}
}
{"mode":"full","isActive":false}


@article{blanchard1957,
  title={Bubble formation and modification in the sea and its meteorological significance},
  author={Blanchard, DCr and Woodcock, AH},
  journal={Tellus},
  volume={9},
  number={2},
  pages={145--158},
  year={1957},
  publisher={Taylor \& Francis}
}
{"mode":"full","isActive":false}






@article{kikuchi2023physico,
  title={Physico-mathematical model for multiple ultrasound-contrast-agent microbubbles encapsulated by a visco-elastic shell: Effect of shell compressibility on ultrasound attenuation},
  author={Kikuchi, Yusei and Kanagawa, Tetsuya and Ayukai, Takahiro},
  journal={Chemical Engineering Science},
  volume={269},
  pages={117541},
  year={2023},
  publisher={Elsevier}
}




@book{Randall1951,
    title = {An introduction to acoustics},
    year = {1951},
    author = {Randall, R. H.},
    publisher = {Dover}
}



